Graphical-model based estimation and inference for differential privacy

Many privacy mechanisms reveal high-level information about a data distribution through noisy measurements. It is common to use this information to estimate the answers to new queries. In this work, we provide an approach to solve this estimation problem efficiently using graphical models, which is particularly effective when the distribution is high-dimensional but the measurements are over low-dimensional marginals. We show that our approach is far more efficient than existing estimation techniques from the privacy literature and that it can improve the accuracy and scalability of many state-of-the-art mechanisms.

==> dan-technical.tex <==
\section{Notation and setup}\label{notation-and-setup}

\subsection{General}\label{general}

\begin{itemize}
\item
  \(\I\{ \cdot \}\) is indicator function.
\item
  \([m] = \{1, 2, \ldots, m\}\) for any integer \(m\)
\end{itemize}

\subsection{Individual data records}\label{individual-data-records}

Single record \(\x = (x_1, \ldots, x_d)\)
\begin{itemize}
\item \(x_i\) is \(i\)th attribute
\item \(x_i\) belongs to domain \(\dom_i\), which is finite with \(n_i\) possible values
\item Overall domain is \(\dom = \prod_{i=1}^d \dom_i\), which has size \(n = \prod_{i=1}^d n_i\). This is exponential in the number of attributes \(d\).
\end{itemize}
  
\subsection{Data set and full contingency
table}\label{data-set-and-full-contingency-table}

\(m\) individuals with records \(\x^{(1)}, \ldots, \x^{(m)}\)

Data set \(\mathbf{X} = (\x^{(1)}, \ldots, \x^{(m)})\)

Contingency table \(\p\) counts the number of individuals with record
equal to \(\x\) for each \(\x\) in the domain. Definition:
\[\p(\x) = \sum_{i=1}^m \I\{\x^{(i)}  = \x\}, \quad \forall \x \in \dom\]

(Convention: use \(\p\) to represent contingency tables because
contingency tables and their marginals behave much like probability
tables and their marginals. The main difference is: contingency tables
are non-negative integers and sum to \(m\); probabilities are
non-negative real numbers and sum to \(1\).)

We will consider \(\p\) to be a vector in \(\R^{n}\) with index set
\(\dom\) (say, ordered lexicographically)

\subsection{Marginals}\label{marginals}

Let \(A \subseteq [d]\) be a generic subset of attributes. Define:

\begin{itemize}
\item
  \(\x_A = (x_i)_{i \in A}\) to be the subvector of \(\x\) restricted to
  attributes in \(A\)
\item
  \(\dom_A = \prod_{i \in A} \dom_i\) be the restricted domain, with
  size \(n_A = \prod_{i \in A} n_i\)
\item
  Let \(-A = [m]\setminus A\) be the complement of \(A\)
\end{itemize}

Define the marignal contingency table (or just ``marginal'') \(\bmu_A\)
as \[
  \bmu_A(\x_A) = \sum_{i=1}^m \I\{ \x^{(i)}_A = \x_A\}
  \]

Note that \(\bmu_A(\x_A)\) is a linear function of \(\p\): \[
  \bmu_A(\x_A) = \sum_{\x_{-A}\in \dom_{-A}} \p(\x_{A}, \x_{-A})
  \] so there exists a matrix \(M_A \in \R^{n_A \times n}\) such that
\(\bmu_A = M_A\p\).

\textbf{(Q: Do you want to use bold or mathbb for matrices?)}

\subsection{Queries}\label{queries}

A linear query is a vector \(\q\) with answer \(\q^T \p\).

A set of \(r\) linear queries \(\q_1, \ldots, \q_r\) can be arranged in
a matrix \(Q \in \R^{r \times n}\) with \(i\)th row equal to \(\q_i\).

The vector of answers to the queries is \(Q \p\).

\(Q\) is the set of \emph{measurement queries}

\subsection{Queries over marginals}\label{queries-over-marginals}

A query may depend only on the marginal table \(\bmu_A\) for a subset
\(A\) of attributes. In this case we write the query as
\(\q_A \in \R^{n_A}\) and the answer is \(\q_A^T \bmu_A\).

(If needed: write \(\q_{A,i}\) if we need to index multiple queries.)

(Optional: A query \(\q\) can be written this way if it can be expressed
as \(\q = M_A^T \q_A\). Then \[
  \q^T \p = \q_A^T M_A \p = \q_A^T \bmu_A
  \] This means \(\q\) is in the row space of \(M_A\). Additional
interpretation?)

\subsection{Measurement cliques}\label{measurement-cliques}

Assume each measurement query depends only on the marginal \(\bmu_C\)
for some \(C \in \C\), where \(\C\) is a collection of cliques (subsets
of attributes). We refer to the collection \(\C\) as the
\emph{measurement cliques}.

There are \(r_C\) total queries for clique \(C\), given in the rows of
the matrix \(Q_C \in \R^{r_C \times n_C}\).

We observe answers \(\y_C = Q_C \bmu_C + \text{Lap}(\Delta_C/\epsilon)\)
for each \(C\). (Check this. Describe sensitivity \(\Delta_C\).)

Let \(\y = (\y_C)_{C \in \C}\) be the complete set of answers to
measurement queries (the concatenation of the query answers from each
clique). Let \(\bmu = (\bmu_C)_{C \in \C}\) be the complete set of
marginals for those cliques.

(Optional: there is a matrix \(M\) such that \(\bmu = M \p\). It is
obtained by stacking the matrices \(M_C\) for all \(C \in \C\).)

\textbf{Observation}: measurements \(\y\) depend only on \(\bmu\), which
is much lower dimensional than \(\p\).

\textbf{Terminology summary} (refine if needed):

\begin{itemize}
\item Measurement cliques \(\C\)
\item Measurement marginals \(\bmu = (\bmu_C)_{C \in \C}\)
\item Measurement queries \(Q = \{Q_C\}_{C \in \C}\)
\item Measurements \(\y = (\y_C)_{C \in \C}\)
\end{itemize}

%\section{Approach}\label{approach}
%
%\subsection{Optimization for
%Estimation}\label{optimization-for-estimation}
%
%We observe \(\y\) (as defined above) and want to answer a target query
%\(\q\). (For now assume we are answering just one arbitrary test query.
%Later we will discuss answering many queries or queries with more
%structure.) We either didn't ask \(\q\) directly, or we did ask it but
%want to use \emph{all} of the available information to estimate
%\(\q^T \p\) as opposed to just using the noisy answer we got.
%
%What principle can we follow? The goal of ``inference'' in DP is to
%estimate \(\hat{\p} \approx \p\) using all available information and
%then use \(\hat{\p}\) to answer later queries. (Cite previous papers.)
%We will refine the terminology to call finding \(\hat{\p}\)
%\emph{estimation}, and using \(\hat{\p}\) to answer the target query
%\emph{inference}. (This matches graphical model terminology.)
%
%The standard framework for estimation and inference uses optimization to
%find \(\hat{\p}\): \[
%\hat{\p}= \argmin_{\p \in \mathcal{S}} F(\p; \y), \qquad \text{answer} = \q^T \hat{\p}
%\]
%
%\begin{itemize}
%\item
%  \(\mathcal{S} = \big\{ \p: \p \geq 0, \mathbf{1}^T \p = m\big\}\) is
%  the (scaled) probability simplex. We relaxed counts from integers to
%  real numbers.
%\item
%  \(F(\p; \y)\) is a loss function. We will usually just write
%  \(F(\p)\).
%\item
%  Examples include L2 and L1
%\item
%  L1 corresponds to a maximum-likelihood criterion
%\item
%  Point out that ``L1'' can use different weights to model MLE when the
%  different queries had different amounts of noise added
%\end{itemize}
%
%\textbf{Problem}: this doesn't scale to high dimensions. The size of
%\(\p\) is exponential in \(d\), and we have to construct it as an
%intermediate step even if the inputs and outputs are small, e.g., if all
%measurement queries and the target query are low-dimensional. (This
%really happens.)
%
%\subsection{Optimization in Terms of
%Marginals}\label{optimization-in-terms-of-marginals}
%
%Assume the loss only depends on measurement marginals \(\bmu\):
%\[
%F(\p; \y) = L(\bmu(\p); \y)
%\]
%
%\begin{itemize}
%\item
%  Again, we will usually just write \(L(\bmu)\)
%\item
%  Examples: L1 or L2 with the measurement queries we described. Give details.
%\item
%  The loss will often have the structure
%  \[ L(\bmu) = \sum_{C \in \C} L_C(\bmu_C)\]
%  but it is not required for our methods.
%\end{itemize}
%
%An ``obvious'' idea would be just to estimate the measurement marginals:
%\[
%\hat{\bmu}= \argmin_{\bmu \in \M} L(\bmu), \qquad \text{answer} = ???
%\]
%
%\begin{itemize}
%\item
%  \(\M = \big\{ \bmu: \exists \p \in \mathcal{S} \text{ with marginals } \bmu \big\}\)
%  is the marginal polytope
%\end{itemize}
%
%The problem with this is that it doesn't tell us how to answer a new
%query, unless that query happens to depend only on some measurement
%marginal \(\bmu_C\).
%
%% I no longer think the next statements are relevant / appropriate.
%%Second, even for queries that are determined by a measurement marginal \(\bmu_C\), it is unclear what criterion is being used to answer the query.
%% For example, the constraint set implies that \emph{some} information from other cliques is being used to estimate \(\bmu_C\), but how, exactly, is this information ``transferred'' to the estimate \(\hat{\bmu}_C\)?
%
%\subsection{\texorpdfstring{Factored \(\p\) and Maximum Entropy
%Criterion}{Factored \textbackslash{}p and Maximum Entropy Criterion}}\label{factored-p-and-maximum-entropy-criterion}
%
%Our solution: we will show that, given a solution
%\(\hat{\bmu} \in \argmin_{\bmu \in \M} L(\bmu)\), we can find a
%distribution \(\hat{\p}\) that has maximum entropy among all
%distributions with marginals \(\hat{\bmu}\). Because it is factored, we
%can represent \(\hat{\p}\) compactly and use it to answer new queries
%efficeintly.
%
%\textbf{Factored distributions (graphical models)}. Let
%\(\p(\x; \btheta) = \frac{1}{Z} \sum_{C \in \C} \exp( \btheta_C(\x_C) )\).
%This distribution is a graphical model that factors over the clique set
%\(\C\). The vector \(\btheta = (\btheta_C)_{C \in \C}\) comprises the
%parameters of the graphical model.
%
%\textbf{Theorem} (imprecise). Let
%\(\hat{\bmu} \in \argmin_{\bmu \in \M} L(\bmu)\). We can compute
%parameters \(\hat{\btheta}(\hat{\bmu})\) such that
%\(p(\x; \hat{\btheta}(\hat{\bmu}))\) has maximum entropy among all
%distributions with marginals \(\hat{\bmu}\). The parameters are not
%uniquely determined by \(\hat{\bmu}\) but the distribution
%\(\p(\x; \hat{\btheta}(\hat{\bmu}))\) is uniquely determined.
%
%\textbf{Technical notes}
%
%\begin{itemize}
%\item
%  As stated this is basically a direct consequence of standard marginal
%  polytope stuff from Wainwright and Jordan (Theorem 3.4 and surrounding
%  content)
%\item
%  There is a technicality: the theorem as stated only applies if
%  \(\hat{\bmu}\) is in the \emph{interior} of the marginal polytope.
%  Specifically this means it has no zeros. We need to figure out what to
%  say if \(\hat{\bmu}\) has zeros. I hope there will be a satisfactory
%  precise statement. Something like: there is a sequence of
%  values\ldots{} (see part (a) of Theorem 3.4).
%\item
%  \textbf{Ideally we'd like a stronger statement}: we can find a
%  factored distribution that has maximum entropy among all distributions
%  with marginals that minimize \(L(\bmu)\). Mathematically it would look
%  something like this: \[
%    \p(\x; \hat{\btheta}) \in \argmax_{\p \in \mathcal{S}} H(\p) \quad \text{s.t. } \, \bmu(\p) \in \argmin_{\bmu \in \M} L(\bmu)
%    \] The reason we don't obviously get this is because if \(L(\bmu)\)
%  has multiple minima, we might choose one minimum \(\hat{\bmu}\) that
%  leads to lower entropy than if we had chosen a different one. If
%  \(L(\bmu)\) is strictly convex, it has a single minimum and we get
%  what we want. There's a chance that we get the stronger property
%  defined by the way we solve the problem (e.g., the proximal method)
%  but this is something we'd have to analyze much more carefully.
%\item
%  TODO: Dan come back and resolve as much of this as possible. Ryan,
%  feel free to take a crack at it if you want.
%\end{itemize}
%
%\section{Algorithms}\label{algorithms}
%
%\subsection{Estimation}\label{estimation}
%
%We need algorithms to find \(\hat{\bmu}\) and \(\hat{\btheta}\). We have
%two approaches, the ``direct method'' (need a better name for this) and
%a proximal method.
%
%\subsubsection{Direct Method}\label{direct-method}
%
%Describe direct method where we parameterize the marginals
%\(\bmu(\btheta)\) as a function of \(\btheta\) and then solve: \[
%\min_{\btheta} L\big( \bmu(\btheta) \big)
%\]
%
%\begin{itemize}
%\item
%  Pro: no constraints
%\item
%  Pro: can compute derivatives etc. using message passing
%\item
%  Con: not convex!
%\end{itemize}
%
%Give as many details as necessary. Cite Domke. Can defer stuff to
%appendix.
%
%\subsubsection{Proximal Method}\label{proximal-method}
%
%Describe proximal method. Directly solve
%\(\argmin_{\bmu \in \M} L(\bmu)\) using a variant of entropic mirror
%descent (or regularized dual averaging?). Cite Vilnis et al.
%
%\begin{itemize}
%\item
%  Pro: convex, guaranteed convergence
%\item
%  Pro: recover \(\hat{\btheta}\) ``for free''
%\item
%  Con: sometimes slower?
%\end{itemize}
%
%\subsection{Inference}\label{inference}
%
%Describe the class of target queries we can support. Give basic
%notation, etc.
%
%Describe the novel variant of variable elimination to compute these
%queries.
%
%\section{Extras}\label{extras}
%
%\subsection{Nonlinear queries}\label{nonlinear-queries}
%
%The method applies to nonlinear queries over marginals. Write a single
%such query as \(\q_A(\bmu_A)\) where \(\q_A: \R^{n_A} \to \R\). Our
%algorithm needs only \(\grad {\q_A}\).
%
%(optional) Write a batch of nonlinear queries as \(Q_A(\bmu_A)\) where
%\(Q_A: \R^{n_A} \to \R^{r_A}\). Our algorithm needs the Jacobian of
%\(Q_A\).
%
%This means \(\q_A\) and \(Q_A\) need to be continuous and
%differentiable.


==> experiments_old.tex <==
\section{Experiments} \label{sec:experiments}

\ry{this section will need to be restructured quite a bit}
\ry{can we combine related work and experiments? As we will compare against related work}
\ry{also, plots are hard to read in black and white}

Next we evaluate empirically the efficiency and accuracy of our proposed methods.  All experiments are performed on a quad-core Intel i7 3.6 GHz processor with 16 GB of RAM.  

For the efficiency experiments, we used synthetic data, allowing us to systematically vary the domain size and number of dimensions of the data and evaluate their impact.  Specifically, we consider a dataset with 1 million tuples and $d$ variables, each with domain size $n_i = 10$. We vary $d = 2 \dots 16 $. We consider chain structured measurements, which include the $\{ i, i+1 \}$ marginals for $ 1 \leq i \leq d-1 $.  

For accuracy experiments, we use the Adult dataset obtained from the UCI machine learning repository \cite{Dua:2017}, which contains 32,561 tuples and 11 discrete (or appropriately discretized) attributes: age, workclass, education, marital status, occupation, relationship to householder, race, sex, hours-per-week, country, and income>=50K.  The total domain size is $ 100 \times 9 \times 16 \times 7 \times 15 \times 6 \times 5 \times 2 \times 100 \times 42 \times 2 \approx 7.6 \times 10^{11} $.  

\begin{figure}[t]
\centering
\subcaptionbox{\label{fig:chain} Model estimation from measurements}{\includegraphics[width=0.45\textwidth]{fig/chain.pdf}}
\subcaptionbox{\label{fig:inference} Target query inference}{\includegraphics[width=0.45\textwidth]{fig/chain_inference.pdf}}
\caption{The runtime of model estimation and inference as dimensionality grows.} \label{fig:efficiency}
\end{figure}


%\ry{I'm wondering if these things can be moved to related work}
% GM: I don't think so, but we could try to shorten if we need to. 

\textbf{Efficiency of estimation.}
Fig. \ref{fig:chain} shows the runtime of our two algorithms for model estimation, Direct and Proximal, compared with two competing methods, LSQR and MW. LSQR \cite{Zhang18Ektelo:} is an iterative algorithm for solving an ordinary least squares problem (without non-negativity constraints); it the most efficient method we are aware of that handles general linear measurements. Least-squares is a very common estimation method in the literature \cite{hay2010boosting,Nikolov13Geometry,li2014data,qardaji2013understanding,ding2011differentially,Xiao10Differential,li2010optimizing}. We use it here to find the minimum-norm $d$-way contingency table which minimizes squared error given the chain-structured measurements.  
%showed that by simply representing the measurements as a sparse matrix and using an iterative conjugate gradient algorithm (such as LSQR) was more efficient in practice.  
MW uses multiplicative weights to repeatedly update an estimate of the full contingency table to reflect the noisy measurements \cite{hardt2012simple}.  While the authors of  \cite{hardt2012simple} describe an enhancement that uses a factored representation, it only applies when the measurements can be partitioned into groups that depend on disjoint subsets of variables.  That enhancement offers no benefit for chain-structured measurements, but would make MW efficient for measurements on disjoint sets of variables.  Nevertheless, our methods do not have such an extreme requirement in order to benefit from the efficiency of a factored representation.

%For measurement sets that can be partitioned in this way, the factored variant of the multiplicative weights algorithm would be more efficient.  Our algorithms would also be efficient in this setting, which shows that our algorithms operate over a factored representation of the data for a more general class of queries than factored multiplicative weights.  

%Although this method can operate on a compact factored representation of $\hat{\p}$ in some cases, for chain-structured measurements it requires materializing the full representation.   

The Direct and Proximal algorithms are both linear in the number of dimensions for chain structured measurements, and as shown in Fig. \ref{fig:chain}, our algorithms are highly scalable, running in a matter of seconds up to $d=16$.  We were unable to run LSQR or MW beyond $d=7$ due to the memory requirements of jointly representing the measurements.  For these methods, the measurements are represented as a sparse matrix, which requires storing $(d-1) \cdot 10^d$ values.  If the measurement queries were represented more compactly, these algorithms may be able to scale up to $d=8$ or $d=9$, but beyond that storing the full contingency table would be impossible on common hardware.


\textbf{Efficiency of inference.}
We now empirically evaluate the inference algorithm we described in Sec.~\ref{inference} to answer factored queries with $\Q_i \in \R^{2 \times n_i}$.  The details of the queries encoded are not important for measuring efficiency, only the size of $\Q_i$ matters.  However, we can interpret this query matrix as compressing the distribution (see supplemental material for more information).    

We compare our inference method (Algorithm~\ref{alg:inference}) to a baseline algorithm that first computes the full contingency table (using the formula from definition~\ref{def:graphical-model}) then answers the queries over the full contingency table.  As shown in Fig. ~\ref{fig:inference}, the baseline breaks down after $ d = 7 $ due to memory limitations, but our algorithm easily scales to $d=16$.   

\textbf{Accuracy of inferred query estimates.}
Next we demonstrate the accuracy improvements afforded by proper inference.  The measurement and target queries, for the Adult dataset, are listed in Fig. ~\ref{table:key}.  There are six carefully chosen low-dimensional query matrices in the measurement set, in addition to the $11$ 1-way marginals (not listed).  The privacy budget of $ \epsilon = 2.0$ is split equally among these $17$ measurement sets.  There are four additional target query matrices.  
The matrix $\P$ in Fig. ~\ref{table:key} contains range queries that characterize the cumulative distribution function, and the matrix $\A$ is a low-sensitivity query matrix from which the answers to range queries can be accurately derived.\cite{li2015matrix} These special query matrices are used for the continuous variables (age and hours-per-week) to demonstrate the important capability of our technology to handle arbitrary measurements of the marginals.
%\ry{for consistency we should consider describing the measurements before the subsections (as we do for chain queries)}

%\gm{below I say 'in-measurement' and 'out-of-measurement' to distinguish the experiments.  Maybe in-clique and out-of-clique are better?}

We evaluate accuracy of our inferred query answers in two settings.  First, we study accuracy on queries that are present in the measurement set (queries 1-6 in Fig.~\ref{table:key}).   Our inferred answers are consistent and incorporate all available evidence.  We compare with a baseline method that simply reports the noisy measurement answer. Second, we study accuracy on queries {\em not} present in the measurement set (queries 7-10 in Fig.~\ref{table:key}).  
%and \gmref{spanning multiple cliques}{I think this point is important: all your measurements are marginals, so there are un-measured queries within cliques, e.g. range queries on a 1-way marginal}.  
Since the first baseline does not apply here, we compare with a different baseline that uses the 1-way marginal measurements and assumes independence among the variables involved in the queries.
%
We used the Proximal algorithm for estimating $\p_{\btheta}$, running it for 2500 iterations (or about 25 seconds) using line search to select the step sizes $t_k$. %Small improvements to accuracy would be possible by running additional iterations. 
We evaluate the quality of a query estimate using the median $L_1$ error over 25 random trials.  The results are shown in Fig. ~\ref{fig:adult1} and ~\ref{fig:adult2}.

\begin{figure}
\centering
\captionsetup{justification=centering}
\subcaptionbox{\label{table:key} Measurement queries (1-6) \\ \hspace{7pt} and target queries (7-10)}{
\resizebox{0.31\textwidth}{!}{%
\begin{tabular}{|c|l|l|}
\hline
\textbf{\#} & \textbf{Clique Variables}                                                      & \textbf{Query Set} \\\hhline{|=|=|=|}
1           & workclass, education                                                           & $\II \otimes \II$              \\
2           & education, income                                                              & $\II \otimes \II$              \\
3           & age, marital status                                                            & $\A \otimes \II$              \\
4           & age, relationship                                                              & $\A \otimes \II$              \\
5           & \begin{tabular}[c]{@{}c@{}}marital status, sex, \\ hours-per-week\end{tabular} & $\II \otimes \II \otimes \A$          \\
6           & race, country                                                                  & $\II \otimes \II$             \\ \hhline{|=|=|=|}
7           & workclass, income                                                              & $\II \otimes \II$              \\
8           & marital status, relationship                                                   & $\II \otimes \II$            \\
9           & relationship, hours-per-week                                                   & $\II \otimes \P$              \\
10          & occupation, sex                                                                & $\II \otimes \II$             \\\hline
\end{tabular}} \vspace{3 mm}
}
\subcaptionbox{\label{fig:adult1} In-measurement \\ \hspace{5pt} target queries}{\includegraphics[width=0.33 \textwidth]{fig/adult1}}
\subcaptionbox{\label{fig:adult2} Out-of-measurement \\ \hspace{-10pt} target queries}{\includegraphics[width=0.33 \textwidth]{fig/adult2}}
\caption{L1 Error from baseline estimates and our estimates.} \label{fig:adult}
\end{figure}

For the in-measurement target queries, we found that our inferred query answers offered lower error than the corresponding baseline on all the measured 2-way and 3-way marginals, usually by a substantial amount.  In result not shown, it also improved the error on 9 out of 11 of the 1-way marginal estimates (the difference in error on the other 2 marginal estimates was negligible).

For the out-of-measurement target queries, our inferred query answers offered meaningful improvements to error for the first three measurements, and a small improvement for the fourth.  This is because the measurement queries contain more information about the first three target queries.  Note that the error of both methods is much worse for out-of-measurement queries because they can not be expressed as a linear combination of the measured queries.  Despite the high error, it is still useful to have better-than-baseline estimates of these quantities.  

Improvements in accuracy stemming from inference have been observed before in the privacy literature (e.g. \cite{hay2010boosting}), however existing inference algorithms are not capable of scaling to the large domain we considered in this experiment.



